Dependence of Dust Formation on the Supernova Explosion

We investigate the properties, composition, and dynamics of dust formation and growth for a diverse set of core-collapse supernovae (CCSNe), varying the progenitor mass, explosion energy, and engine type. These explosions are evolved with a 1-D Lagrangian hydrodynamics code out to several hundred days to model the ejecta as it expands and cools. A multigrain dust nucleation and growth model is applied to these results. We find that higher explosion energies lead to an earlier onset of dust formation, smaller grain sizes, and larger silicate abundances. Further, we see that nuclear burning during the explosion leads to enhanced formation of silicate dust. Finally, we build composite models from our suite to predict the efficiency of CCSNe dust production as a function of metallicity.

==> Tables/Mejecta.tex <==
\begin{deluxetable}{c|cccccc}
\tablecaption{Ejecta masses for aSNe and HNe
\label{tab:Mejecta}}
\tablehead{\colhead{Type} & \colhead{f} & \colhead{$\Theta$} & \colhead{$M_{ejecta,cone}$} & \colhead{$E_{exp,cone}$}  & \colhead{$M_{ejecta,rest}$} & \colhead{$E_{exp,rest}$}\\
 & fit & viewing angle & $\mathrm{M}_{\odot}$ & $\mathrm{foe}$ & $\mathrm{M}_{\odot}$ & $\mathrm{foe}$}
\colnumbers
\startdata
aSN & 3 & 40 & 0.117 & 4.65  & 0.883 & 0.52 \\
aSN & 2 & 20 & 0.030 & 3.67  & 0.970 & 0.92 \\
aSN & 5 & 20 & 0.030 & 14.50 & 0.970 & 0.58 \\
HN  & - & 15  & 0.034 & 14.80 & 0.966 & 4.65 \\
HN  & - & 10  & 0.015 & 18.40 & 0.985 & 4.79 \\
HN  & - & 40  & 0.234 & 18.40 & 0.766 & 0.91 \\
\enddata
\tablecomments{The aSN ejecta estimates are formulated for a 1 foe symmetric explosion, whereas the HN ejecta estimates are formulated using a 5 foe symmetric explosion. LEAVING IN UNTIL I'M DONE WITH REFERENCING VALUES.}
\end{deluxetable}
